Variational Inference with Tail-adaptive f-Divergence

Variational inference with {\alpha}-divergences has been widely used in modern probabilistic machine learning. Compared to Kullback-Leibler (KL) divergence, a major advantage of using {\alpha}-divergences (with positive {\alpha} values) is their mass-covering property. However, estimating and optimizing {\alpha}-divergences require to use importance sampling, which could have extremely large or infinite variances due to heavy tails of importance weights. In this paper, we propose a new class of tail-adaptive f-divergences that adaptively change the convex function f with the tail of the importance weights, in a way that theoretically guarantees finite moments, while simultaneously achieving mass-covering properties. We test our methods on Bayesian neural networks, as well as deep reinforcement learning in which our method is applied to improve a recent soft actor-critic (SAC) algorithm. Our results show that our approach yields significant advantages compared with existing methods based on classical KL and {\alpha}-divergences.

==> tex/rebuttal.tex <==
\textbf{Rebuttal for ``Variational Inference with Tail Adapted \emph{f}-Divergence''}
\vspace{6pt}

%We highly appreciate the time and valuable comments from all the reviewers, all of which we will take into serious consideration in our revision. 
We thank all the reviewers for their valuable comments. 

\textbf{\#Reviewer 1} \newline
We thank Reviewer \#1 for the comments.  We will fix the typos and improve the writing in the final version. 

\vspace{6pt}
\textbf{\#Reviewer 3} \newline
Thank you for your time and thorough feedback.  
We will provide detailed proofs of proposition 4.1 and proposition 5.1 in our revision. 
Here we give the brief outlines of the proof. 

\begin{proof}[Proof of Proposition 4.1 (a)]
Recall that $f(t) = (at+b) + \int_0^\infty (t-\mu)_+ h(\mu)d\mu$. Calculation shows 
$$
f'(t) = a + \int_0^t h(\mu) d\mu, ~~~f''(t) = h(t).
$$
Since $h$ is non-negative, we have $f(t)$ is convex. Conversely, by specifying $f''(t) = h(t)$,
we can represent any convex function in the form above. %convex function.
% $$
% \begin{aligned}
% D_f (p || q_\theta) &= \E_{q_\theta}\bigg[ f(\frac{p}{q})- f(1)\bigg ] \\
% &= \E_{q_\theta} \bigg[ at+ b - (a +b) + \int_0^\infty (t-\mu)_+ f^{''}(\mu) - \int_0^\infty (1-\mu)_+ f^{''}(\mu)\bigg] \\
% &= \int_0^\infty f^{''}(\mu)\E_{q_\theta}\bigg[ \bigg(\frac{p}{q} - \mu\bigg)_+\bigg] + \red{some ~constant?}
% \end{aligned}
% $$
\end{proof}

\begin{proof}[Proof of Proposition 5.1] Recall that $\bar F_w(t) = \prob(w  > t)$. We have $\nabla \bar F_w(t) = q_w(t)$, where $q_w$ is the density of random variable $w$. 
$$
\E_{q_w}[\bar F^{\beta}_w] =  \int q_w(t) \bar F^{\beta}_w(t)  dt = \int\bar F^\beta_w(t) d \bar F_\beta(t) = \int_{0}^1 t^{\beta} dt,$$ 
which is finite only when $\beta >-1$. 
In addition, we have $\phi_{w,\beta}(t) \sim t^{-\beta\alpha*}$ directly following the definition of the tail index (see Line 99-102). 
 
%Let $\{x_i\}$ be draws from $q$, and $w_i=p(x_i)/q(x_i)$ with cumulative distribution function
%$F_w(t)= 1 - \bar{F}_{w}(t)$ defined by $\bar{F}_w(t)=\text{Pr}(w>t)$.
%such that for some $\alpha^*>0$, 
%$$
%\bar{F}_w(t) = t^{\alpha^*}L(t).
%% E_q[ \phi_{w,\beta}(w)] = w^{-1/\gamma}L(x)~~ \text{for}~w>0,
%$$
%where $-\alpha^*$ is called the tail index, and $L$ is slowly varying function satisfying $ \lim_{t\rightarrow \infty} \frac{L(tx)}{L(t)} = 1. $
%\red{cite xxx}, we have $\E_q[t^{\alpha*}] < \infty$ and hence 
%$$ \E_q[t^{\alpha}] < \infty, ~~~ \forall \alpha= -\beta \alpha_*  < \alpha* ~~\text{for any}~\beta > -1.$$
\end{proof}

\vspace{6pt}
\textbf{\#Reviewer 4} \newline
Thank you for your time and your valuable comments. 

* ``In proposition 5.1, with respect to what distribution, the expectation is taken? p or q? '' \newline
- The expectation is taken w.r.t. $q$.

* ``The proposition 5.1 only states the bounded mean. Since authors talked about estimation variance of alpha divergence, I thought the second order moment of phi(ratio) might be more interesting than the mean? '' \newline
- By setting $\beta>-0.5$, we would be able to guarantee finite variance of importance weights (while $\beta > -1$ guarantees finite mean). However, our experiments show taking  $\beta=-1$ normally yields the best empirical performance. 
This could be because an infinite variance is somehow a less serious problem than an infinite mean, 
and we want to use the most negative $\beta$ while keeping finite mean. 
%
In fact, perhaps counter-intuitively, it can be shown theoretically that stochastic gradient descent with infinite variance can still converge (see T. P. Krasulina 1969. On Stochastic  Approximation Processes with Infinite Variance); 
but it's impossible to establish convergence with an infinite mean (since the objective itself it is not well defined!).  
%would the whole optimization %
%studies show 

* ``What is the estimation variance of the gradient in Algorithm 1? How does it compare with the alpha divergence? '' \newline
- Estimating the exact value of the variance of the gradient is computational and theoretically difficult. But it is expected that it is generally much more stable than $\alpha$ divergence,  because the weights we introduce are rank-based and never scale exponentially like $\alpha$-divergence. 
As we point out earlier, the bigger issue is that $\alpha$ divergence may not even exist if $\alpha$ is larger than the tail index of ratio $p(x)/q(x)$ (which is very difficult to check in practice). 

We will clarify these issues in our revised version. Thanks again for your comments. 
%We find that alpha-divergences tend to have degenerate importance weights,the phenomenon is also reported in `Li et al. 2016 Renyi', which may lead to high-variances of the gradient estimator, however, our approach replaces the f function with a rank function which provides more stable importance weights and gradient estimates.


% It's widely known that alpha-divergences 
% which leads to high-variance of gradient estimator. However, our approach with


==> tex/related.tex <==

\section{Related Work}


